RoMa: Robust Dense Feature Matching

Feature matching is an important computer vision task that involves estimating correspondences between two images of a 3D scene, and dense methods estimate all such correspondences. The aim is to learn a robust model, i.e., a model able to match under challenging real-world changes. In this work, we propose such a model, leveraging frozen pretrained features from the foundation model DINOv2. Although these features are significantly more robust than local features trained from scratch, they are inherently coarse. We therefore combine them with specialized ConvNet fine features, creating a precisely localizable feature pyramid. To further improve robustness, we propose a tailored transformer match decoder that predicts anchor probabilities, which enables it to express multimodality. Finally, we propose an improved loss formulation through regression-by-classification with subsequent robust regression. We conduct a comprehensive set of experiments that show that our method, RoMa, achieves significant gains, setting a new state-of-the-art. In particular, we achieve a 36% improvement on the extremely challenging WxBS benchmark. Code is provided at https://github.com/Parskatt/RoMa

==> dedode_short.tex <==
\section{Steering DeDoDe~Descriptions}

\begin{figure*}
    \centering
    \includegraphics[width=0.8\linewidth]{figures/dedode-rot/rot1.png}
    \includegraphics[width=0.8\linewidth]{figures/dedode-rot/W1rot1.png}
    \caption{\textbf{Steering DeDoDe~descriptions under quarter turn rotations.} In the top image pair we match the ordinary descriptions. In the bottom image pair we instead modify the descriptions of the keypoints in the right image by multiplying them by a steering matrix $W$.}
    \label{fig:steer-rot1}
\end{figure*}
\begin{figure*}
    \centering
    \includegraphics[width=0.9\linewidth]{figures/dedode-rot/rot2.png}
    \includegraphics[width=0.9\linewidth]{figures/dedode-rot/W2rot2.png}
    \caption{\textbf{Steering DeDoDe~descriptions under half turn rotations.} In the top image pair we match the ordinary descriptions. In the bottom image pair we instead modify the descriptions of the keypoints in the right image by multiplying them by a steering matrix $W^2$.}
    \label{fig:steer-rot2}
\end{figure*}
\begin{figure*}
    \centering
    \includegraphics[width=0.8\linewidth]{figures/dedode-rot/rot3.png}
    \includegraphics[width=0.8\linewidth]{figures/dedode-rot/W3rot3.png}
    \caption{\textbf{Steering DeDoDe~descriptions under three-quarter turn rotations.} In the top image pair we match the ordinary descriptions. In the bottom image pair we instead modify the descriptions of the keypoints in the right image by multiplying them by a steering matrix $W^3$.}
    \label{fig:steer-rot3}
\end{figure*}

As noted in \cite{edstedt2023dedode}, DeDoDe~is not rotation invariant.
Here we propose a simple technique for improving matching under large in-plane rotations.
The underlying assumption, which will be empirically proven, is that DeDoDe~descriptions are rotation equivariant rather than invariant.
Concretely, we assume that there exists a matrix \mbox{$W\in\mathbb{R}^{256\times 256}$} (here $256$ is the dimension of the descriptions), such that for a trained descriptor network $\mathbf{g}_\theta$ we have
\begin{equation}\label{eq:steer}
    \mathbf{g}_\theta(R_{90}\mathbf{x}^{\mathrm{kp}} | \mathtt{rot}(I)) \approx W\mathbf{g}_\theta(\mathbf{x}|I),
\end{equation}
where $R_{90}$ is a quarter turn rotation matrix, rotating the keypoints about the center of the image and $\mathtt{rot}$ rotates an image a quarter turn.
In other words, when we rotate the input to $\mathbf{g}_\theta$,
the output descriptions are (approximately) transformed by multiplication with $W$.
We then say that $\mathbf{g}_\theta$ is equivariant and that $W$ steers the descriptions $\mathbf{g}_\theta(\mathbf{x}^\mathrm{kp} | I)$.
Note that it is far from obvious that such $W$ should exist
as we do not enforce this in any way during training of $\mathbf{g}_\theta$,
we do not even use rotation augmentation.

Given the trained detector and descriptor networks --- which we keep fixed --- we wish to find $W$ such that \eqref{eq:steer} holds.
Remarkably, simply training $W$ on the MegaDepth training set with the $L_1$-loss
\begin{equation}
    \left\|\mathbf{g}_\theta(R_{90}^k\mathbf{x}^{\mathrm{kp}} | \mathtt{rot}^k(I)) - W^k\mathbf{g}_\theta(\mathbf{x}|I)\right\|_1
\end{equation}
seems to work well.
Here, the number of rotations $k$ is sampled from $\{1, 2, 3\}$ for each training batch.
Once we have obtained $W$, we can match rotated images by simply
multiplying the descriptions by $W^k$.
We demonstrate this in Figures~\ref{fig:steer-rot1}, \ref{fig:steer-rot2}, \ref{fig:steer-rot3}.

Finally, investigations into implicitly learned equivariance in networks have
focused more or less exclusively on networks trained for image classification \cite{Lenc_2015_CVPR,gruver2023the,Bruintjes_2023_CVPR,bökman2023investigating}.
Therefore we believe that the finding
of a high degree of equivariance in the DeDoDe~descriptor can inspire future research on learned equivariance for models trained on a diversity of tasks.



==> preamble.tex <==
%
% --- inline annotations
%
\usepackage[dvipsnames, table]{xcolor}
\newcommand{\red}[1]{{\color{red}#1}}
%\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}


\RequirePackage{times}    % Integrate Times for here
\RequirePackage{xspace}
\RequirePackage{graphicx}
\RequirePackage{amsmath}
\RequirePackage{amssymb}
\RequirePackage{booktabs}
\RequirePackage[numbers,sort&compress]{natbib}

\usepackage{tikz}
\usepackage[style=english]{csquotes}
\usepackage[detect-all,per-mode=symbol,group-digits=integer,group-minimum-digits=4,group-separator={,}]{siunitx}
\newcommand{\parsection}[1]{\vspace{0mm}\noindent\textbf{#1}~}
\usepackage{todonotes}
\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator*{\argmax}{argmax}

\newcommand{\ours}[0]{RoMa}
\newcommand{\B}[0]{\ensuremath{\mathcal{B}}}
\newcommand{\A}[0]{\ensuremath{\mathcal{A}}}

